MadAgents

We uncover an effective and communicative set of agents working with MadGraph. Agentic installation, learning-by-doing training, and user support provide easy access to state-of-the-art simulations and accelerate LHC research. We show in detail how MadAgents interact with inexperienced and advanced users, support a range of simulation tasks, and analyze the results. In a second step, we illustrate how MadAgents automatize event generation and run an autonomous simulation campaign, starting from a pdf file of a paper. We also present successive MadAgents updates, including a Claude Code implementation with a self-improvement loop.

==> md-cache/5a9603164a587e7211959776206a7e6c.md.tex <==
\markdownRendererDocumentBegin
\markdownRendererSectionBegin
\markdownRendererHeadingOne{Tutorial 5: BSM Effective Field Theories in MadGraph}\markdownRendererInterblockSeparator
{}In this tutorial you will extend the Standard Model simulations you have already performed to include Beyond-the-Standard-Model (BSM) effects described by Effective Field Theories (EFTs). EFTs add higher-dimensional operators to the Standard Model, weighted by \markdownRendererStrongEmphasis{Wilson coefficients} that parameterize possible new physics at scales beyond direct reach.\markdownRendererParagraphSeparator
{}You will learn how to:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Import an EFT UFO model into MadGraph5\markdownRendererUnderscore{}aMC@NLO (MG5\markdownRendererUnderscore{}aMC).\markdownRendererUlItemEnd 
\markdownRendererUlItem Identify EFT-specific parameters (Wilson coefficients) in \markdownRendererCodeSpan{param\markdownRendererUnderscore{}card.dat}.\markdownRendererUlItemEnd 
\markdownRendererUlItem Generate simple LHC processes (such as Drell–Yan–like channels) with EFT contributions at parton level.\markdownRendererUlItemEnd 
\markdownRendererUlItem Organize multiple runs corresponding to different EFT parameter points in preparation for later Simulation-Based Inference (SBI) studies.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}\markdownRendererBlockQuoteBegin
\markdownRendererStrongEmphasis{Important:} Treat this tutorial directory as read-only instructions. Do all your own work, models, cards, scripts, and runs in:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererCodeSpan{/output/tutorials/my\markdownRendererUnderscore{}work/05\markdownRendererUnderscore{}bsm\markdownRendererUnderscore{}eft\markdownRendererUnderscore{}models}\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererBlockQuoteEnd \markdownRendererInterblockSeparator
{}You can consult this \markdownRendererCodeSpan{README.md} at any time while working in your own area.\markdownRendererInterblockSeparator
{}\markdownRendererThematicBreak{}\markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererHeadingTwo{1. Prerequisites}\markdownRendererInterblockSeparator
{}Before starting this tutorial, you should:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Have completed Tutorials 1–4:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem MG5 basics and the MG5 → Pythia → Delphes pipeline.\markdownRendererUlItemEnd 
\markdownRendererUlItem Standard Model Drell–Yan generation at parton level.\markdownRendererUlItemEnd 
\markdownRendererUlItem Pythia showering and hadronization.\markdownRendererUlItemEnd 
\markdownRendererUlItem Delphes detector simulation.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererUlItemEnd 
\markdownRendererUlItem Be comfortable with:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Defining and generating processes in MG5.\markdownRendererUlItemEnd 
\markdownRendererUlItem Locating and editing \markdownRendererCodeSpan{run\markdownRendererUnderscore{}card.dat} and \markdownRendererCodeSpan{param\markdownRendererUnderscore{}card.dat}.\markdownRendererUlItemEnd 
\markdownRendererUlItem Running Pythia and Delphes via MG5’s run interface (conceptually, you will still focus mainly on the hard-scattering stage here).\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererUlItemEnd 
\markdownRendererUlItem Have a basic conceptual understanding of EFTs:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem The idea of extending the Standard Model Lagrangian with higher-dimensional operators.\markdownRendererUlItemEnd 
\markdownRendererUlItem The role of Wilson coefficients as parameters controlling the strength of these operators.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}All practical work for this tutorial should be carried out in:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererCodeSpan{/output/tutorials/my\markdownRendererUnderscore{}work/05\markdownRendererUnderscore{}bsm\markdownRendererUnderscore{}eft\markdownRendererUnderscore{}models}\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}\markdownRendererThematicBreak{}\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingTwo{2. UFO models and EFTs in MG5}\markdownRendererInterblockSeparator
{}MG5 uses \markdownRendererStrongEmphasis{UFO models} (Universal FeynRules Output) to encode the particle content, interactions, and parameters of a theory. A UFO model typically provides:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem A list of particles (including any new states).\markdownRendererUlItemEnd 
\markdownRendererUlItem A set of parameters (masses, couplings, mixing angles, Wilson coefficients, etc.).\markdownRendererUlItemEnd 
\markdownRendererUlItem The interaction vertices needed to build amplitudes.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererHeadingThree{2.1 Standard Model vs. EFT-extended models}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem The default Standard Model implementation (e.g. \markdownRendererCodeSpan{sm}) contains only Standard Model particles and parameters.\markdownRendererUlItemEnd 
\markdownRendererUlItem An EFT-extended UFO model adds \markdownRendererStrongEmphasis{new parameters} that represent coefficients of higher-dimensional operators, often denoted symbolically as \markdownRendererInlineMath{C_i} or similar.\markdownRendererUlItemEnd 
\markdownRendererUlItem In many EFT models, no new light particles are introduced; instead, the new physics manifests through modified interactions among existing Standard Model fields.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{2.2 Importing an EFT UFO model}\markdownRendererInterblockSeparator
{}To use an EFT model, you first need a UFO implementation installed in a location MG5 can see (for example, inside the \markdownRendererCodeSpan{models/} directory of your MG5 installation or in a path you configure explicitly). The exact model name and installation procedure depend on your local setup and chosen EFT.\markdownRendererParagraphSeparator
{}At the MG5 prompt, you typically import the model via:\markdownRendererInterblockSeparator
{}\markdownRendererInputFencedCode{md-cache/02abdd2f7ef8c1803c3d398d95608907.verbatim}{text}{text}\markdownRendererInterblockSeparator
{}Here \markdownRendererCodeSpan{MODEL\markdownRendererUnderscore{}NAME} is a placeholder for the EFT UFO model you have installed. Examples in the literature include SMEFT-like models or simplified contact-interaction models, but this tutorial remains agnostic about the specific choice.\markdownRendererParagraphSeparator
{}Once imported, you can inspect the model’s content:\markdownRendererInterblockSeparator
{}\markdownRendererInputFencedCode{md-cache/f23201a06176d946913930a115144941.verbatim}{text}{text}\markdownRendererInterblockSeparator
{}Look for new parameters and interactions compared to the pure Standard Model.\markdownRendererInterblockSeparator
{}\markdownRendererThematicBreak{}\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd 
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingTwo{3. EFT parameters and \markdownRendererCodeSpan{param\markdownRendererUnderscore{}card.dat}}\markdownRendererInterblockSeparator
{}The \markdownRendererStrongEmphasis{param card} (\markdownRendererCodeSpan{param\markdownRendererUnderscore{}card.dat}) in a process directory stores numerical values for all model parameters, including any EFT additions.\markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererHeadingThree{3.1 Locating EFT parameters (Wilson coefficients)}\markdownRendererInterblockSeparator
{}After importing an EFT model and generating a process (see Section 4), MG5 will create a process directory with a \markdownRendererCodeSpan{Cards/param\markdownRendererUnderscore{}card.dat}. Inside this file, you should find:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Standard Model parameters (masses, gauge couplings, etc.).\markdownRendererUlItemEnd 
\markdownRendererUlItem Additional parameters corresponding to EFT operators (e.g. Wilson coefficients), usually grouped into dedicated blocks.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}You can identify EFT parameters by:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Reading block names and comments in \markdownRendererCodeSpan{param\markdownRendererUnderscore{}card.dat}.\markdownRendererUlItemEnd 
\markdownRendererUlItem Comparing with the model’s documentation to understand which operators each parameter controls.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{3.2 Modifying EFT parameters}\markdownRendererInterblockSeparator
{}There are two common ways to change EFT parameter values:\markdownRendererInterblockSeparator
{}\markdownRendererOlBegin
\markdownRendererOlItemWithNumber{1}\markdownRendererStrongEmphasis{Editing \markdownRendererCodeSpan{param\markdownRendererUnderscore{}card.dat} directly}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Open \markdownRendererCodeSpan{Cards/param\markdownRendererUnderscore{}card.dat} in a text editor.\markdownRendererUlItemEnd 
\markdownRendererUlItem Locate the block and entries corresponding to the parameters you want to modify.\markdownRendererUlItemEnd 
\markdownRendererUlItem Change the numerical values as desired.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{2}\markdownRendererStrongEmphasis{Using MG5 \markdownRendererCodeSpan{set param\markdownRendererUnderscore{}card} commands} (when supported)\markdownRendererInterblockSeparator
{}\markdownRendererUlBegin
\markdownRendererUlItem Within the MG5 run interface, you can often use commands like:\markdownRendererInterblockSeparator
{}\markdownRendererInputFencedCode{md-cache/9711108e3f93677c19f07c08ae17be69.verbatim}{text}{text}\markdownRendererInterblockSeparator
{}where \markdownRendererCodeSpan{NAME} and \markdownRendererCodeSpan{INDEX} identify the parameter and \markdownRendererCodeSpan{VALUE} is the new numerical value.\markdownRendererUlItemEnd 
\markdownRendererUlItem The exact syntax and availability depend on the model and MG5 version; use \markdownRendererCodeSpan{help set} within MG5 for details.\markdownRendererUlItemEnd 
\markdownRendererUlEnd \markdownRendererOlItemEnd 
\markdownRendererOlEnd \markdownRendererInterblockSeparator
{}In this tutorial, you do \markdownRendererStrongEmphasis{not} need any specific “correct” values for EFT parameters. Instead, you will pick a few representative settings (keeping them within modest ranges suggested by the model documentation) and compare the resulting event samples qualitatively.\markdownRendererInterblockSeparator
{}\markdownRendererBlockQuoteBegin
\markdownRendererStrongEmphasis{Note:} Always keep track of which param card you used for each run. Saving copies of \markdownRendererCodeSpan{param\markdownRendererUnderscore{}card.dat} with descriptive filenames can help you later when building SBI datasets.\markdownRendererBlockQuoteEnd \markdownRendererInterblockSeparator
{}\markdownRendererThematicBreak{}\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd 
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingTwo{4. Simple EFT processes at the LHC}\markdownRendererInterblockSeparator
{}To connect with your earlier work, you can consider processes where EFT operators modify familiar Standard Model channels.\markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererHeadingThree{4.1 Drell–Yan–like processes}\markdownRendererInterblockSeparator
{}EFT operators can alter dilepton production at the LHC, for example in processes of the form\markdownRendererParagraphSeparator
{}\markdownRendererDisplayMath{p p \to \ell^+ \ell^- + X,}\markdownRendererParagraphSeparator
{}where new four-fermion or gauge–fermion operators modify the kinematics or overall rates compared to the pure Standard Model.\markdownRendererParagraphSeparator
{}Using an EFT UFO model, you can define a Drell–Yan–like process similarly to the Standard Model case, but with the EFT model active:\markdownRendererInterblockSeparator
{}\markdownRendererInputFencedCode{md-cache/a68a4fb01ec26ea2f7ecb45197df4705.verbatim}{text}{text}\markdownRendererInterblockSeparator
{}Here \markdownRendererCodeSpan{MODEL\markdownRendererUnderscore{}NAME} stands for your chosen EFT model. The process definition is structurally similar to the Standard Model Drell–Yan case, but now EFT interactions are available in the amplitude.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{4.2 Other illustrative processes}\markdownRendererInterblockSeparator
{}Depending on your EFT model, other channels might be interesting:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Diboson production, e.g. \markdownRendererInlineMath{p p \to W^+ W^- + X}.\markdownRendererUlItemEnd 
\markdownRendererUlItem Contact-interaction–like processes involving jets and leptons.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}You can define such processes in the same way, using \markdownRendererCodeSpan{generate} with the EFT model imported.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{4.3 Workflow summary}\markdownRendererInterblockSeparator
{}A typical EFT simulation workflow at parton level is:\markdownRendererInterblockSeparator
{}\markdownRendererOlBeginTight
\markdownRendererOlItemWithNumber{1}Start MG5 and import the EFT model.\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{2}Define any multiparticle labels (e.g. \markdownRendererCodeSpan{p}, \markdownRendererCodeSpan{l+}, \markdownRendererCodeSpan{l-}).\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{3}Generate the process of interest.\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{4}Output the process directory.\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{5}Inspect and modify \markdownRendererCodeSpan{Cards/param\markdownRendererUnderscore{}card.dat} to set EFT parameters.\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{6}Launch parton-level runs (and, if desired, subsequent Pythia and Delphes steps) using \markdownRendererCodeSpan{launch}.\markdownRendererOlItemEnd 
\markdownRendererOlEndTight \markdownRendererInterblockSeparator
{}You can then compare EFT-deformed samples to their Standard Model counterparts following similar steps but using the Standard Model model file.\markdownRendererInterblockSeparator
{}\markdownRendererThematicBreak{}\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd 
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingTwo{5. Parameter scans and organizing multiple runs}\markdownRendererInterblockSeparator
{}In many EFT studies, you are interested not just in a single point in parameter space, but in how observables change as Wilson coefficients vary.\markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererHeadingThree{5.1 Conceptual view of a parameter scan}\markdownRendererInterblockSeparator
{}A simple parameter scan might involve:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Choosing one or more EFT parameters (e.g. one coefficient \markdownRendererInlineMath{C} and possibly additional ones).\markdownRendererUlItemEnd 
\markdownRendererUlItem Selecting a set of parameter points (different choices of \markdownRendererInlineMath{C} values) that sample a range of interest.\markdownRendererUlItemEnd 
\markdownRendererUlItem Generating event samples for each parameter point under consistent simulation settings (beam energy, cuts, PDFs, shower and detector configurations).\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}The objective is to build a collection of samples that can later be turned into SBI-ready datasets, where each sample is labeled by its underlying parameter values.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{5.2 Organizing multiple runs}\markdownRendererInterblockSeparator
{}There are several ways to organize multiple EFT runs. For example:\markdownRendererInterblockSeparator
{}\markdownRendererUlBegin
\markdownRendererUlItem \markdownRendererStrongEmphasis{Single process directory with multiple runs}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Use one process directory (e.g. \markdownRendererCodeSpan{EFT\markdownRendererUnderscore{}DY\markdownRendererUnderscore{}ll}).\markdownRendererUlItemEnd 
\markdownRendererUlItem For each parameter point, copy or edit \markdownRendererCodeSpan{param\markdownRendererUnderscore{}card.dat} and launch a new run with a distinct run label.\markdownRendererUlItemEnd 
\markdownRendererUlItem Keep a record of which param card corresponds to each run (e.g. by saving a copy in a dedicated subdirectory).\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{Multiple process directories}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Create separate process directories for different parameter configurations or for SM vs. EFT comparisons.\markdownRendererUlItemEnd 
\markdownRendererUlItem This can make bookkeeping simpler but may duplicate code and increase disk usage.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererUlItemEnd 
\markdownRendererUlEnd \markdownRendererInterblockSeparator
{}Whichever approach you choose, it is important to:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Maintain a clear naming scheme that encodes which EFT parameters were used.\markdownRendererUlItemEnd 
\markdownRendererUlItem Store param cards and run logs alongside event files.\markdownRendererUlItemEnd 
\markdownRendererUlItem Record random seeds and software versions when possible.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{5.3 Metadata for later analysis}\markdownRendererInterblockSeparator
{}For future SBI work, you will want to know, for each event sample:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Which process and model were used.\markdownRendererUlItemEnd 
\markdownRendererUlItem Which EFT parameters (and their values) were active.\markdownRendererUlItemEnd 
\markdownRendererUlItem Which run card settings (e.g. cuts, beam energy) were applied.\markdownRendererUlItemEnd 
\markdownRendererUlItem Which versions of MG5, Pythia, and Delphes were used.\markdownRendererUlItemEnd 
\markdownRendererUlItem How many events were generated and which random seeds were used.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}A simple way to capture this information is to create a lightweight metadata file (for example, in JSON or YAML format) in each run directory, summarizing the key settings. You will formalize this further in Tutorial 6.\markdownRendererInterblockSeparator
{}\markdownRendererThematicBreak{}\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd 
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingTwo{6. Exercises (no solutions or numeric answers in this file)}\markdownRendererInterblockSeparator
{}Carry out all hands-on tasks in your own workspace:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererCodeSpan{/output/tutorials/my\markdownRendererUnderscore{}work/05\markdownRendererUnderscore{}bsm\markdownRendererUnderscore{}eft\markdownRendererUnderscore{}models}\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}This \markdownRendererCodeSpan{README.md} provides prompts only. It does not contain solutions, numeric answers, or fully worked command files.\markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererHeadingThree{Exercise 1 – Importing an EFT model and inspecting its content}\markdownRendererInterblockSeparator
{}\markdownRendererOlBeginTight
\markdownRendererOlItemWithNumber{1}Install or locate an EFT UFO model accessible to your MG5 installation.\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{2}In MG5, use \markdownRendererCodeSpan{import model} to load this EFT model.\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{3}Use \markdownRendererCodeSpan{display particles}, \markdownRendererCodeSpan{display parameters}, and \markdownRendererCodeSpan{display interactions} to identify:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Any new particles compared to the Standard Model.\markdownRendererUlItemEnd 
\markdownRendererUlItem New parameters that correspond to EFT operators or Wilson coefficients.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{4}In your notes, summarize how the EFT model extends the Standard Model content.\markdownRendererOlItemEnd 
\markdownRendererOlEndTight \markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{Exercise 2 – Generating an EFT-extended Drell–Yan–like process}\markdownRendererInterblockSeparator
{}\markdownRendererOlBeginTight
\markdownRendererOlItemWithNumber{1}Using your EFT model, define multiparticle labels for proton beams and leptons.\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{2}Generate a Drell–Yan–like process (e.g. with an oppositely charged lepton pair in the final state) using the EFT model.\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{3}Output the process to a new directory in your work area and inspect the \markdownRendererCodeSpan{Cards/param\markdownRendererUnderscore{}card.dat} file.\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{4}Identify which parameters in \markdownRendererCodeSpan{param\markdownRendererUnderscore{}card.dat} correspond to EFT operators that can affect your chosen process.\markdownRendererOlItemEnd 
\markdownRendererOlEndTight \markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{Exercise 3 – Varying one EFT parameter and comparing samples}\markdownRendererInterblockSeparator
{}\markdownRendererOlBeginTight
\markdownRendererOlItemWithNumber{1}Choose one EFT parameter (for example, a single Wilson coefficient) that is relevant for your process.\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{2}Define a small set of distinct parameter choices for this coefficient.\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{3}For each choice, modify \markdownRendererCodeSpan{param\markdownRendererUnderscore{}card.dat} accordingly and run a parton-level simulation (and optionally Pythia and Delphes).\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{4}Compare the resulting samples qualitatively, focusing on how selected observables (such as dilepton invariant mass or angular distributions) appear to change.\markdownRendererOlItemEnd 
\markdownRendererOlEndTight \markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{Exercise 4 – Organizing runs and naming conventions}\markdownRendererInterblockSeparator
{}\markdownRendererOlBeginTight
\markdownRendererOlItemWithNumber{1}Design a naming scheme for process directories and run labels that encodes:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem The process type (e.g. Drell–Yan).\markdownRendererUlItemEnd 
\markdownRendererUlItem The EFT model name.\markdownRendererUlItemEnd 
\markdownRendererUlItem The values (or labels) of the EFT parameters used.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{2}Apply this scheme consistently to the runs you produced in Exercises 2 and 3.\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{3}Create a short documentation file in your work area that explains the naming convention and how to interpret each component.\markdownRendererOlItemEnd 
\markdownRendererOlEndTight \markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{Exercise 5 – Extending to additional processes}\markdownRendererInterblockSeparator
{}\markdownRendererOlBeginTight
\markdownRendererOlItemWithNumber{1}Choose a second process (for example, a diboson or contact-interaction–like channel) where your EFT model is expected to have an impact.\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{2}Generate EFT-extended events for this process using at least two different EFT parameter settings.\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{3}Compare, in qualitative terms, how the EFT effects manifest differently in this process compared to the Drell–Yan–like case.\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{4}Update your run organization and naming scheme to accommodate multiple processes.\markdownRendererOlItemEnd 
\markdownRendererOlEndTight \markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{Exercise 6 – Planning for SBI datasets}\markdownRendererInterblockSeparator
{}\markdownRendererOlBeginTight
\markdownRendererOlItemWithNumber{1}Based on your EFT runs, list the key pieces of information you would want recorded in a metadata file for each sample (e.g. process name, model name, EFT parameters, run card settings, number of events, seeds).\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{2}Sketch, in a text document or pseudocode, how you would automatically generate such metadata files after each run.\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{3}Reflect on how this metadata will help when you later prepare datasets for SBI in Tutorial 6.\markdownRendererOlItemEnd 
\markdownRendererOlEndTight \markdownRendererInterblockSeparator
{}\markdownRendererThematicBreak{}\markdownRendererInterblockSeparator
{}By completing this tutorial, you will have learned how to incorporate EFT UFO models into MG5, control EFT parameters via \markdownRendererCodeSpan{param\markdownRendererUnderscore{}card.dat}, and organize multiple runs across parameter space. These skills are essential for building EFT-aware datasets suitable for Simulation-Based Inference.
\markdownRendererSectionEnd 
\markdownRendererSectionEnd 
\markdownRendererSectionEnd \markdownRendererDocumentEnd

==> md-cache/9b75a80ea0d821fdecca71e638cb1618.md.tex <==
\markdownRendererDocumentBegin
\markdownRendererSectionBegin
\markdownRendererHeadingOne{UFO EFT \markdownRendererInlineMath{pp \to t\bar t} dataset documentation}\markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererHeadingTwo{1. Introduction and overview}\markdownRendererInterblockSeparator
{}This document describes a simulated dataset of effective-field-theory (EFT) top–antitop production at the LHC, including detector effects at Delphes level. The central artifact is the NumPy archive\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererCodeSpan{/output/dataset/output/dataset/ufo\markdownRendererUnderscore{}ttbar\markdownRendererUnderscore{}reweighted.npz}\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}which contains \markdownRendererInlineMath{N = 100000} events with reconstructed jets, electrons, muons, missing transverse energy (MET), and per-event weights.\markdownRendererParagraphSeparator
{}The hard-process signal is \markdownRendererInlineMath{pp \to t\bar t} at \markdownRendererInlineMath{\sqrt{s} = 13\,\text{TeV}}, generated with MadGraph5\markdownRendererUnderscore{}aMC@NLO (MG5\markdownRendererUnderscore{}aMC), interfaced to Pythia8 for parton showering and hadronization, and Delphes 3 for fast detector simulation. An EFT dimension-6 chromomagnetic operator with Wilson coefficient \markdownRendererInlineMath{c_{tG}} is activated in the UFO model \markdownRendererCodeSpan{dim6top\markdownRendererUnderscore{}LO\markdownRendererUnderscore{}UFO}. The parton-level EFT sample is generated at leading order (LO) in QCD and then reweighted with an \markdownRendererInlineMath{m_{t\bar t}}-dependent \markdownRendererInlineMath{K}-factor extracted from Standard Model (SM) LO and next-to-leading order (NLO) \markdownRendererInlineMath{t\bar t} samples.\markdownRendererParagraphSeparator
{}This documentation aims to make the dataset reproducible and interpretable for particle-physics PhD students and practitioners. It covers\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem the software environment and recommended installation,\markdownRendererUlItemEnd 
\markdownRendererUlItem the physics setup and modeling assumptions,\markdownRendererUlItemEnd 
\markdownRendererUlItem the event-generation and reweighting pipeline from hard process to NPZ file,\markdownRendererUlItemEnd 
\markdownRendererUlItem the structure and meaning of each NPZ field, and\markdownRendererUlItemEnd 
\markdownRendererUlItem verification steps and known limitations.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingTwo{2. Software environment and installation}\markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererHeadingThree{2.1 Generator stack (explicit information)}\markdownRendererInterblockSeparator
{}The dataset was produced with the following generator stack and tools. Items marked "explicit" are read directly from configuration files and logs.\markdownRendererInterblockSeparator
{}\markdownRendererUlBegin
\markdownRendererUlItem \markdownRendererStrongEmphasis{MadGraph5\markdownRendererUnderscore{}aMC@NLO core} (explicit)\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Version: 3.7.0.\markdownRendererUlItemEnd 
\markdownRendererUlItem Evidence: \markdownRendererCodeSpan{/opt/MG5\markdownRendererUnderscore{}aMC/VERSION} and the banner at the top of \markdownRendererCodeSpan{/output/dataset/output/log.txt}.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{MadGraph template versions} (explicit)\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem LO and UFO processes (\markdownRendererCodeSpan{proc\markdownRendererUnderscore{}sm\markdownRendererUnderscore{}lo\markdownRendererUnderscore{}ttbar}, \markdownRendererCodeSpan{proc\markdownRendererUnderscore{}ufo\markdownRendererUnderscore{}parton\markdownRendererUnderscore{}ttbar}): \markdownRendererCodeSpan{TemplateVersion.txt = 2.5.0}.\markdownRendererUlItemEnd 
\markdownRendererUlItem NLO process (\markdownRendererCodeSpan{proc\markdownRendererUnderscore{}sm\markdownRendererUnderscore{}nlo\markdownRendererUnderscore{}ttbar}): \markdownRendererCodeSpan{TemplateVersion.txt = 2.4.31}.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{LHAPDF} (explicit)\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Interface version: 6.5.5.\markdownRendererUlItemEnd 
\markdownRendererUlItem Evidence: MG5 log messages ("Using LHAPDF v6.5.5 interface for PDFs"), and \markdownRendererCodeSpan{lhapdf-config --version} under \markdownRendererCodeSpan{/opt/MG5\markdownRendererUnderscore{}aMC/HEPTools/lhapdf6\markdownRendererUnderscore{}py3}.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{Pythia8} (semi-explicit)\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Installed under \markdownRendererCodeSpan{/opt/MG5\markdownRendererUnderscore{}aMC/HEPTools/pythia8}.\markdownRendererUlItemEnd 
\markdownRendererUlItem The installation log refers to unpacking \markdownRendererCodeSpan{pythia8316}, consistent with Pythia 8.316.\markdownRendererUlItemEnd 
\markdownRendererUlItem Exact minor version is not recorded in the dataset area but is expected to be 8.316.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{Delphes} (semi-explicit)\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Installed under \markdownRendererCodeSpan{/opt/MG5\markdownRendererUnderscore{}aMC/Delphes}.\markdownRendererUlItemEnd 
\markdownRendererUlItem The README describes installation from \markdownRendererCodeSpan{Delphes-3.5.0.tar.gz}, consistent with Delphes version 3.5.0.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{MG5–Pythia8 interface} (explicit)\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Path: \markdownRendererCodeSpan{/opt/MG5\markdownRendererUnderscore{}aMC/HEPTools/MG5aMC\markdownRendererUnderscore{}PY8\markdownRendererUnderscore{}interface}.\markdownRendererUlItemEnd 
\markdownRendererUlItem Registered in \markdownRendererCodeSpan{/opt/MG5\markdownRendererUnderscore{}aMC/input/mg5\markdownRendererUnderscore{}configuration.txt} and in the UFO process card.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{UFO model} (explicit)\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Name: \markdownRendererCodeSpan{dim6top\markdownRendererUnderscore{}LO\markdownRendererUnderscore{}UFO}.\markdownRendererUlItemEnd 
\markdownRendererUlItem Location: \markdownRendererCodeSpan{/opt/MG5\markdownRendererUnderscore{}aMC/models/dim6top\markdownRendererUnderscore{}LO\markdownRendererUnderscore{}UFO}.\markdownRendererUlItemEnd 
\markdownRendererUlItem Used in \markdownRendererCodeSpan{mg5\markdownRendererUnderscore{}ufo\markdownRendererUnderscore{}parton\markdownRendererUnderscore{}ttbar.mg5} via \markdownRendererCodeSpan{import model /opt/MG5\markdownRendererUnderscore{}aMC/models/dim6top\markdownRendererUnderscore{}LO\markdownRendererUnderscore{}UFO}.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererUlItemEnd 
\markdownRendererUlEnd \markdownRendererInterblockSeparator
{}All three MG5 processes (SM LO, SM NLO, and EFT UFO) use LHAPDF with \markdownRendererCodeSpan{pdlabel = lhapdf} and PDF set ID \markdownRendererCodeSpan{lhaid = 303400}.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{2.2 Python environment (inferred)}\markdownRendererInterblockSeparator
{}The analysis and conversion scripts are Python 3 programs. In the current container, the environment is:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererStrongEmphasis{Python:} 3.11.2 (inferred via \markdownRendererCodeSpan{python3 --version}).\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{NumPy:} \markdownRendererCodeSpan{numpy==2.3.5} (inferred).\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{Awkward Array:} \markdownRendererCodeSpan{awkward==2.8.11} (inferred).\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{Uproot:} originally installed for the generation run, but the exact version is not recorded. A modern version compatible with Python 3.11, NumPy 2.x, and Awkward 2.x (for example \markdownRendererCodeSpan{uproot\markdownRendererTilde{}=5.3}) is recommended for reproduction.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}These library versions are not guaranteed to match exactly those used in the original run but are physically compatible. Exact bitwise reproducibility is therefore not guaranteed, but physics-level reproducibility (distributions and cross sections within statistical uncertainties) is expected.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{2.3 Clean-machine installation recipe (recommended)}\markdownRendererInterblockSeparator
{}This subsection presents a concrete installation recipe for a new Linux machine. Paths can be adapted as needed; the original project assumes\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem MG5\markdownRendererUnderscore{}aMC at \markdownRendererCodeSpan{/opt/MG5\markdownRendererUnderscore{}aMC}, and\markdownRendererUlItemEnd 
\markdownRendererUlItem the project directory at \markdownRendererCodeSpan{/output/dataset}.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}If these locations are not writable, you can install elsewhere and either adjust the paths in \markdownRendererCodeSpan{run.sh} and the \markdownRendererCodeSpan{.mg5} cards or create suitable symbolic links.\markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererHeadingFour{2.3.1 System prerequisites (example for Debian/Ubuntu)}\markdownRendererInterblockSeparator
{}\markdownRendererInputFencedCode{md-cache/1dbd1ac22555b841207230c2614f25b9.verbatim}{bash}{bash}\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingFour{2.3.2 Python virtual environment for analysis}\markdownRendererInterblockSeparator
{}\markdownRendererInputFencedCode{md-cache/53dcfe158ec104d7de5690155fb56fd9.verbatim}{bash}{bash}\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingFour{2.3.3 Install MG5\markdownRendererUnderscore{}aMC 3.7.0 and HEP tools}\markdownRendererInterblockSeparator
{}\markdownRendererInputFencedCode{md-cache/72c938850fda7e7ce7830a750c5bc8a8.verbatim}{bash}{bash}\markdownRendererInterblockSeparator
{}This will populate\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererCodeSpan{/opt/MG5\markdownRendererUnderscore{}aMC/HEPTools/lhapdf6\markdownRendererUnderscore{}py3},\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererCodeSpan{/opt/MG5\markdownRendererUnderscore{}aMC/HEPTools/pythia8},\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererCodeSpan{/opt/MG5\markdownRendererUnderscore{}aMC/Delphes}, and\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererCodeSpan{/opt/MG5\markdownRendererUnderscore{}aMC/HEPTools/MG5aMC\markdownRendererUnderscore{}PY8\markdownRendererUnderscore{}interface},\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}and will update \markdownRendererCodeSpan{/opt/MG5\markdownRendererUnderscore{}aMC/input/mg5\markdownRendererUnderscore{}configuration.txt} with the appropriate paths for Pythia8 and the interface.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingFour{2.3.4 Install the UFO model \markdownRendererCodeSpan{dim6top\markdownRendererUnderscore{}LO\markdownRendererUnderscore{}UFO}}\markdownRendererInterblockSeparator
{}\markdownRendererInputFencedCode{md-cache/5d14fff1cb3a7d9cee15077388a55fe4.verbatim}{bash}{bash}\markdownRendererInterblockSeparator
{}Verify that the directory \markdownRendererCodeSpan{/opt/MG5\markdownRendererUnderscore{}aMC/models/dim6top\markdownRendererUnderscore{}LO\markdownRendererUnderscore{}UFO} exists and contains UFO model files such as \markdownRendererCodeSpan{particles.py}, \markdownRendererCodeSpan{parameters.py}, \markdownRendererCodeSpan{vertices.py}, etc.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingFour{2.3.5 Place this project}\markdownRendererInterblockSeparator
{}\markdownRendererInputFencedCode{md-cache/f595e5b92b4d28f292dbac58ed5d8a7f.verbatim}{bash}{bash}\markdownRendererInterblockSeparator
{}If you choose a different root (for example \markdownRendererCodeSpan{\markdownRendererDollarSign{}HOME/ufo\markdownRendererUnderscore{}ttbar\markdownRendererUnderscore{}dataset} instead of \markdownRendererCodeSpan{/output/dataset}), update the hard-coded paths in \markdownRendererCodeSpan{run.sh} and in the \markdownRendererCodeSpan{.mg5} cards or provide suitable symlinks.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd 
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{2.4 Explicit vs inferred versions}\markdownRendererInterblockSeparator
{}For clarity:\markdownRendererInterblockSeparator
{}\markdownRendererUlBegin
\markdownRendererUlItem \markdownRendererStrongEmphasis{Explicit versions (from logs/configs):}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem MG5\markdownRendererUnderscore{}aMC core 3.7.0, template versions 2.5.0 (LO/UFO) and 2.4.31 (NLO).\markdownRendererUlItemEnd 
\markdownRendererUlItem LHAPDF 6.5.5.\markdownRendererUlItemEnd 
\markdownRendererUlItem Pythia8 approximately 8.316 (from installation log).\markdownRendererUlItemEnd 
\markdownRendererUlItem Delphes 3.5.0 (from README).\markdownRendererUlItemEnd 
\markdownRendererUlItem UFO model \markdownRendererCodeSpan{dim6top\markdownRendererUnderscore{}LO\markdownRendererUnderscore{}UFO} (exact internal version not specified in the dataset area).\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{Inferred Python environment:}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Python 3.11.2, NumPy 2.3.5, Awkward 2.8.11.\markdownRendererUlItemEnd 
\markdownRendererUlItem Uproot: any recent 5.x compatible with the above; exact original version unknown.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererUlItemEnd 
\markdownRendererUlEnd \markdownRendererInterblockSeparator
{}Exact bitwise reproduction of the dataset is not guaranteed, but reproductions with the versions above should agree within statistical uncertainties.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd 
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingTwo{3. Physics and modeling assumptions}\markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererHeadingThree{3.1 Processes and models}\markdownRendererInterblockSeparator
{}Three MG5 processes are used in the pipeline:\markdownRendererInterblockSeparator
{}\markdownRendererOlBegin
\markdownRendererOlItemWithNumber{1}\markdownRendererStrongEmphasis{SM LO \markdownRendererInlineMath{pp \to t\bar t}}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Card: \markdownRendererCodeSpan{scripts/mg5\markdownRendererUnderscore{}sm\markdownRendererUnderscore{}lo\markdownRendererUnderscore{}ttbar.mg5}.\markdownRendererUlItemEnd 
\markdownRendererUlItem Model: \markdownRendererCodeSpan{sm} (Standard Model).\markdownRendererUlItemEnd 
\markdownRendererUlItem Process: \markdownRendererCodeSpan{generate p p > t t\markdownRendererTilde{}}.\markdownRendererUlItemEnd 
\markdownRendererUlItem Beam energies: \markdownRendererCodeSpan{ebeam1 = ebeam2 = 6500\markdownRendererBackslash{},\markdownRendererBackslash{}text\markdownRendererLeftBrace{}GeV\markdownRendererRightBrace{}} (\markdownRendererInlineMath{\sqrt{s} = 13\,\text{TeV}}).\markdownRendererUlItemEnd 
\markdownRendererUlItem PDFs: \markdownRendererCodeSpan{pdlabel = lhapdf}, \markdownRendererCodeSpan{lhaid = 303400}.\markdownRendererUlItemEnd 
\markdownRendererUlItem Perturbative order: LO QCD (no loop tags).\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{2}\markdownRendererStrongEmphasis{SM NLO \markdownRendererInlineMath{pp \to t\bar t}}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Card: \markdownRendererCodeSpan{scripts/mg5\markdownRendererUnderscore{}sm\markdownRendererUnderscore{}nlo\markdownRendererUnderscore{}ttbar.mg5}.\markdownRendererUlItemEnd 
\markdownRendererUlItem Model: \markdownRendererCodeSpan{sm}.\markdownRendererUlItemEnd 
\markdownRendererUlItem Process: \markdownRendererCodeSpan{generate p p > t t\markdownRendererTilde{} [QCD]} (NLO QCD corrections via aMC@NLO).\markdownRendererUlItemEnd 
\markdownRendererUlItem Same collider and PDF settings as LO.\markdownRendererUlItemEnd 
\markdownRendererUlItem Perturbative order: NLO QCD in fixed-order, no-shower mode.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{3}\markdownRendererStrongEmphasis{EFT UFO \markdownRendererInlineMath{pp \to t\bar t} with dim-6 operator}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Card: \markdownRendererCodeSpan{scripts/mg5\markdownRendererUnderscore{}ufo\markdownRendererUnderscore{}parton\markdownRendererUnderscore{}ttbar.mg5}.\markdownRendererUlItemEnd 
\markdownRendererUlItem Model: \markdownRendererCodeSpan{dim6top\markdownRendererUnderscore{}LO\markdownRendererUnderscore{}UFO} via \markdownRendererCodeSpan{import model /opt/MG5\markdownRendererUnderscore{}aMC/models/dim6top\markdownRendererUnderscore{}LO\markdownRendererUnderscore{}UFO}.\markdownRendererUlItemEnd 
\markdownRendererUlItem Process: \markdownRendererCodeSpan{generate p p > t t\markdownRendererTilde{} FCNC=0 DIM6=1}.\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererCodeSpan{FCNC = 0} disables flavor-changing neutral current operators.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererCodeSpan{DIM6 = 1} activates dimension-6 contributions.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererUlItemEnd 
\markdownRendererUlItem Collider and PDFs: same 13 TeV setup, \markdownRendererCodeSpan{pdlabel = lhapdf}, \markdownRendererCodeSpan{lhaid = 303400}.\markdownRendererUlItemEnd 
\markdownRendererUlItem EFT-specific setting: \markdownRendererCodeSpan{set ctG 1.0} (non-zero chromomagnetic top–gluon operator coefficient in the model’s normalization).\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererOlItemEnd 
\markdownRendererOlEnd \markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{3.2 Top-quark parameters}\markdownRendererInterblockSeparator
{}From the param cards (\markdownRendererCodeSpan{Cards/param\markdownRendererUnderscore{}card.dat}):\markdownRendererInterblockSeparator
{}\markdownRendererUlBegin
\markdownRendererUlItem \markdownRendererStrongEmphasis{SM LO and NLO samples}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Top mass: \markdownRendererInlineMath{m_t = 173\,\text{GeV}}.\markdownRendererUlItemEnd 
\markdownRendererUlItem Yukawa: \markdownRendererInlineMath{y_t = 173\,\text{GeV}} (in SM convention).\markdownRendererUlItemEnd 
\markdownRendererUlItem Width: \markdownRendererInlineMath{\Gamma_t \approx 1.49\,\text{GeV}}.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{EFT UFO sample}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Top mass: \markdownRendererInlineMath{m_t = 172\,\text{GeV}}.\markdownRendererUlItemEnd 
\markdownRendererUlItem Yukawa: \markdownRendererInlineMath{y_t = 172\,\text{GeV}}.\markdownRendererUlItemEnd 
\markdownRendererUlItem Width: \markdownRendererInlineMath{\Gamma_t \approx 1.51\,\text{GeV}}.\markdownRendererUlItemEnd 
\markdownRendererUlItem DIM6 block (excerpt): the EFT scale parameter is set to \markdownRendererInlineMath{\lambda = 1\,\text{TeV}}, and among the listed Wilson coefficients only \markdownRendererInlineMath{c_{tG}} is non-zero; all other entries in that block are set to zero.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererUlItemEnd 
\markdownRendererUlEnd \markdownRendererInterblockSeparator
{}This introduces a small mismatch between the SM reference samples and the EFT UFO sample in \markdownRendererInlineMath{m_t} and \markdownRendererInlineMath{\Gamma_t}, which is acceptable for many use cases but should be kept in mind for precision studies.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{3.3 K-factor construction in \markdownRendererInlineMath{m_{t\bar t}}}\markdownRendererInterblockSeparator
{}To approximate NLO QCD effects for the EFT sample, a one-dimensional \markdownRendererInlineMath{K}-factor in the invariant mass of the top pair \markdownRendererInlineMath{m_{t\bar t}} is constructed.\markdownRendererParagraphSeparator
{}For each LO or NLO SM event, top and anti-top four-vectors are reconstructed from the LHE records. If \markdownRendererInlineMath{p_t = (E_t, \vec p_t)} and \markdownRendererInlineMath{p_{\bar t} = (E_{\bar t}, \vec p_{\bar t})}, then\markdownRendererParagraphSeparator
{}\markdownRendererDisplayMath{
m_{t\bar t} = \sqrt{(E_t + E_{\bar t})^2 - \lVert \vec p_t + \vec p_{\bar t} \rVert^2} \,.
}\markdownRendererParagraphSeparator
{}Events are binned into \markdownRendererInlineMath{N_\text{bins} = 60} uniform bins in \markdownRendererInlineMath{m_{t\bar t} \in [m_\text{min}, m_\text{max}]} with\markdownRendererParagraphSeparator
{}\markdownRendererDisplayMath{
m_\text{min} = 340\,\text{GeV}, \quad m_\text{max} = 2000\,\text{GeV},
}\markdownRendererParagraphSeparator
{}and edges\markdownRendererParagraphSeparator
{}\markdownRendererDisplayMath{
m_i = m_\text{min} + i\,\Delta m, \quad \Delta m = \frac{m_\text{max} - m_\text{min}}{N_\text{bins}}, \quad i = 0, \dots, N_\text{bins}.
}\markdownRendererParagraphSeparator
{}If \markdownRendererInlineMath{N^i_\text{LO}} and \markdownRendererInlineMath{N^i_\text{NLO}} denote the number of events in bin \markdownRendererInlineMath{i} for the LO and NLO SM samples, respectively, then the bin-wise \markdownRendererInlineMath{K}-factors are defined as\markdownRendererParagraphSeparator
{}\markdownRendererDisplayMath{
K_i = \begin{cases}
\dfrac{N^i_\text{NLO}}{N^i_\text{LO}} & \text{if } N^i_\text{LO} > 0, \\
1 & \text{if } N^i_\text{LO} = 0.\end{cases}
}\markdownRendererParagraphSeparator
{}Events with \markdownRendererInlineMath{m_{t\bar t}} outside \markdownRendererInlineMath{[m_\text{min}, m_\text{max}]} are ignored in the histogram and do not affect the \markdownRendererInlineMath{K_i}.\markdownRendererParagraphSeparator
{}The resulting array of edges \markdownRendererInlineMath{\{m_i\}} and values \markdownRendererInlineMath{\{K_i\}} is stored in JSON format as \markdownRendererCodeSpan{kfactors\markdownRendererUnderscore{}mtt.json}.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{3.4 Application of \markdownRendererInlineMath{K(m_{t\bar t})} to EFT UFO events}\markdownRendererInterblockSeparator
{}For the EFT UFO sample, \markdownRendererInlineMath{m_{t\bar t}} is reconstructed per event using the first top and anti-top found in the LHE records (by PDG IDs \markdownRendererInlineMath{+6} and \markdownRendererInlineMath{-6}). The \markdownRendererInlineMath{K}-factor is then applied piecewise:\markdownRendererParagraphSeparator
{}\markdownRendererDisplayMath{
K(m_{t\bar t}) = \begin{cases}
K_0, & m_{t\bar t} < m_0, \\
K_i, & m_i \le m_{t\bar t} < m_{i+1}, \\
K_{N_\text{bins}-1}, & m_{t\bar t} \ge m_{N_\text{bins}}.\end{cases}
}\markdownRendererParagraphSeparator
{}The new event weight is defined as\markdownRendererParagraphSeparator
{}\markdownRendererDisplayMath{
w_\text{new}(m_{t\bar t}) = w_\text{orig}\,K(m_{t\bar t}),
}\markdownRendererParagraphSeparator
{}where \markdownRendererInlineMath{w_\text{orig}} is the original weight from the UFO LHE file. Negative weights (if present) are preserved in sign and scaled in magnitude.\markdownRendererParagraphSeparator
{}The script \markdownRendererCodeSpan{scripts/apply\markdownRendererUnderscore{}kfactor\markdownRendererUnderscore{}to\markdownRendererUnderscore{}lhe.py} performs this transformation and writes a CSV file \markdownRendererCodeSpan{ufo\markdownRendererUnderscore{}event\markdownRendererUnderscore{}weights.csv} with columns\markdownRendererParagraphSeparator
{}\markdownRendererDisplayMath{
(\text{ievt},\, m_{t\bar t},\, K(m_{t\bar t}),\, w_\text{orig},\, w_\text{new}).
}\markdownRendererParagraphSeparator
{}Note that events with \markdownRendererInlineMath{m_{t\bar t}} outside \markdownRendererInlineMath{[m_\text{min}, m_\text{max}]} are assigned \markdownRendererInlineMath{K_0} or \markdownRendererInlineMath{K_{N_\text{bins}-1}} as above, not \markdownRendererInlineMath{K=1}.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{3.5 Approximations and assumptions}\markdownRendererInterblockSeparator
{}Key modeling assumptions:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem The EFT UFO sample is generated at LO in QCD; NLO QCD effects are approximated by a one-dimensional \markdownRendererInlineMath{K(m_{t\bar t})} derived from SM LO and NLO samples.\markdownRendererUlItemEnd 
\markdownRendererUlItem The \markdownRendererInlineMath{K}-factor depends only on \markdownRendererInlineMath{m_{t\bar t}}, assuming that higher-order QCD corrections factorize and can be well approximated by a function of \markdownRendererInlineMath{m_{t\bar t}} alone.\markdownRendererUlItemEnd 
\markdownRendererUlItem The same \markdownRendererInlineMath{K(m_{t\bar t})} is applied to the EFT process with \markdownRendererInlineMath{c_{tG} \ne 0}, assuming that NLO QCD corrections factorize similarly in the presence of this operator.\markdownRendererUlItemEnd 
\markdownRendererUlItem SM and EFT samples have slightly different \markdownRendererInlineMath{m_t} and \markdownRendererInlineMath{\Gamma_t}, which may induce small inconsistencies in the mapping.\markdownRendererUlItemEnd 
\markdownRendererUlItem Background processes such as \markdownRendererInlineMath{W}+jets, single top, and QCD multijets are not included in this dataset; it contains only the EFT \markdownRendererInlineMath{t\bar t} signal.\markdownRendererUlItemEnd 
\markdownRendererUlItem Detector effects are modeled with Delphes 3.5.0 using a standard MG5-supplied card, not a full GEANT-based simulation, and no pileup.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}These approximations are acceptable for many new-physics sensitivity and machine-learning studies, but the dataset should not be used as a precision reference for full NLO+PS+EW phenomenology.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd 
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingTwo{4. Generation pipeline (from hard process to NPZ)}\markdownRendererInterblockSeparator
{}This section summarizes the full pipeline orchestrated by \markdownRendererCodeSpan{/output/dataset/run.sh}.\markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererHeadingThree{4.1 SM LO and NLO generation}\markdownRendererInterblockSeparator
{}\markdownRendererOlBegin
\markdownRendererOlItemWithNumber{1}\markdownRendererStrongEmphasis{SM NLO \markdownRendererInlineMath{pp \to t\bar t}}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem MG5 card: \markdownRendererCodeSpan{scripts/mg5\markdownRendererUnderscore{}sm\markdownRendererUnderscore{}nlo\markdownRendererUnderscore{}ttbar.mg5}.\markdownRendererUlItemEnd 
\markdownRendererUlItem Output directory: \markdownRendererCodeSpan{/output/dataset/output/proc\markdownRendererUnderscore{}sm\markdownRendererUnderscore{}nlo\markdownRendererUnderscore{}ttbar} (with run name \markdownRendererCodeSpan{sm\markdownRendererUnderscore{}nlo}).\markdownRendererUlItemEnd 
\markdownRendererUlItem Settings:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererCodeSpan{ebeam1 = ebeam2 = 6500\markdownRendererBackslash{},\markdownRendererBackslash{}text\markdownRendererLeftBrace{}GeV\markdownRendererRightBrace{}}.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererCodeSpan{pdlabel = lhapdf}, \markdownRendererCodeSpan{lhaid = 303400}.\markdownRendererUlItemEnd 
\markdownRendererUlItem Dynamical scales with \markdownRendererCodeSpan{fixed\markdownRendererUnderscore{}ren\markdownRendererUnderscore{}scale = fixed\markdownRendererUnderscore{}fac\markdownRendererUnderscore{}scale = False}, \markdownRendererCodeSpan{dynamical\markdownRendererUnderscore{}scale\markdownRendererUnderscore{}choice = -1} (default MG5 dynamic scale), and reference scales \markdownRendererCodeSpan{\markdownRendererBackslash{}mu\markdownRendererUnderscore{}R\markdownRendererCircumflex{}\markdownRendererBackslash{}text\markdownRendererLeftBrace{}ref\markdownRendererRightBrace{} = \markdownRendererBackslash{}mu\markdownRendererUnderscore{}F\markdownRendererCircumflex{}\markdownRendererBackslash{}text\markdownRendererLeftBrace{}ref\markdownRendererRightBrace{} \markdownRendererBackslash{}approx 91.1\markdownRendererBackslash{},\markdownRendererBackslash{}text\markdownRendererLeftBrace{}GeV\markdownRendererRightBrace{}}.\markdownRendererUlItemEnd 
\markdownRendererUlItem No parton shower in this step (\markdownRendererCodeSpan{shower=OFF} in the card, and run in "noshower" mode).\markdownRendererUlItemEnd 
\markdownRendererUlItem Generator-level cuts: minimal jet transverse momentum of 10 GeV (\markdownRendererCodeSpan{ptj = 10}), minimal photon transverse momentum of 20 GeV (\markdownRendererCodeSpan{ptgmin = 20}), and no explicit \markdownRendererInlineMath{\eta} cuts on jets or leptons (\markdownRendererCodeSpan{etaj = -1}, \markdownRendererCodeSpan{etal = -1}).\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{2}\markdownRendererStrongEmphasis{SM LO \markdownRendererInlineMath{pp \to t\bar t}}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem MG5 card: \markdownRendererCodeSpan{scripts/mg5\markdownRendererUnderscore{}sm\markdownRendererUnderscore{}lo\markdownRendererUnderscore{}ttbar.mg5}.\markdownRendererUlItemEnd 
\markdownRendererUlItem Output directory: \markdownRendererCodeSpan{/output/dataset/output/proc\markdownRendererUnderscore{}sm\markdownRendererUnderscore{}lo\markdownRendererUnderscore{}ttbar} (run name \markdownRendererCodeSpan{sm\markdownRendererUnderscore{}lo}).\markdownRendererUlItemEnd 
\markdownRendererUlItem Settings: same collider and PDF configuration as NLO, LO matrix elements, and no explicit generator-level \markdownRendererInlineMath{p_T} or \markdownRendererInlineMath{\eta} cuts beyond MG5 defaults.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererOlItemEnd 
\markdownRendererOlEnd \markdownRendererInterblockSeparator
{}Both SM samples use a 4-flavor scheme (\markdownRendererCodeSpan{maxjetflavor = 4} in the LO and UFO run cards), treating \markdownRendererInlineMath{b} as heavier than the maximum jet flavor.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{4.2 K-factor construction}\markdownRendererInterblockSeparator
{}The script \markdownRendererCodeSpan{scripts/build\markdownRendererUnderscore{}kfactor\markdownRendererUnderscore{}mtt.py} is called with\markdownRendererInterblockSeparator
{}\markdownRendererInputFencedCode{md-cache/25a79e3fc90f9deb811acf121cc8d6e5.verbatim}{bash}{bash}\markdownRendererInterblockSeparator
{}It automatically locates the relevant LHE files in the \markdownRendererCodeSpan{Events/} subdirectories, reconstructs \markdownRendererInlineMath{m_{t\bar t}} per event, fills LO and NLO histograms, and computes \markdownRendererInlineMath{K_i} as described in Section 3.3. The resulting JSON is later used to reweight the EFT UFO sample.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{4.3 EFT UFO generation}\markdownRendererInterblockSeparator
{}The EFT process \markdownRendererCodeSpan{pp \markdownRendererBackslash{}to t\markdownRendererBackslash{}bar t} with \markdownRendererCodeSpan{DIM6=1} and \markdownRendererCodeSpan{FCNC=0} is generated using\markdownRendererInterblockSeparator
{}\markdownRendererInputFencedCode{md-cache/677abe65004984e5c30e9d7949063fc2.verbatim}{text}{text}\markdownRendererInterblockSeparator
{}with key lines:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererCodeSpan{import model /opt/MG5\markdownRendererUnderscore{}aMC/models/dim6top\markdownRendererUnderscore{}LO\markdownRendererUnderscore{}UFO}.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererCodeSpan{generate p p > t t\markdownRendererTilde{} FCNC=0 DIM6=1}.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererCodeSpan{set ctG 1.0}.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererCodeSpan{set ebeam1 6500}, \markdownRendererCodeSpan{set ebeam2 6500}.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererCodeSpan{set pdlabel lhapdf}, \markdownRendererCodeSpan{set lhaid 303400}.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}MG5 outputs to \markdownRendererCodeSpan{/output/dataset/output/proc\markdownRendererUnderscore{}ufo\markdownRendererUnderscore{}parton\markdownRendererUnderscore{}ttbar} with run name \markdownRendererCodeSpan{ufo\markdownRendererUnderscore{}parton}, producing an unweighted UFO LHE file at parton level.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{4.4 Reweighting UFO events}\markdownRendererInterblockSeparator
{}The script \markdownRendererCodeSpan{scripts/apply\markdownRendererUnderscore{}kfactor\markdownRendererUnderscore{}to\markdownRendererUnderscore{}lhe.py} is then used to apply the \markdownRendererInlineMath{m_{t\bar t}}-dependent \markdownRendererInlineMath{K}-factor to the UFO events:\markdownRendererInterblockSeparator
{}\markdownRendererInputFencedCode{md-cache/6fccacc06c208ad96d8219a2ff4edae6.verbatim}{bash}{bash}\markdownRendererInterblockSeparator
{}The resulting reweighted LHE file replaces the original UFO LHE, and \markdownRendererCodeSpan{ufo\markdownRendererUnderscore{}event\markdownRendererUnderscore{}weights.csv} records \markdownRendererInlineMath{(\text{ievt}, m_{t\bar t}, K, w_\text{orig}, w_\text{new})} for each event.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{4.5 Pythia8 shower and Delphes detector simulation}\markdownRendererInterblockSeparator
{}\markdownRendererCodeSpan{run.sh} then:\markdownRendererInterblockSeparator
{}\markdownRendererOlBegin
\markdownRendererOlItemWithNumber{1}Ensures MG5 configuration values for Pythia8 and the MG5aMC–Pythia interface are set in \markdownRendererCodeSpan{me5\markdownRendererUnderscore{}configuration.txt} under \markdownRendererCodeSpan{proc\markdownRendererUnderscore{}ufo\markdownRendererUnderscore{}parton\markdownRendererUnderscore{}ttbar/Cards}.\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{2}Selects a Delphes card by copying the first matching \markdownRendererCodeSpan{delphes\markdownRendererUnderscore{}card*.dat} from\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererCodeSpan{/opt/MG5\markdownRendererUnderscore{}aMC/Template/Cards/} or\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererCodeSpan{/opt/MG5\markdownRendererUnderscore{}aMC/Template/Common/Cards/}\markdownRendererSoftLineBreak
{}into \markdownRendererCodeSpan{/output/dataset/output/proc\markdownRendererUnderscore{}ufo\markdownRendererUnderscore{}parton\markdownRendererUnderscore{}ttbar/Cards/delphes\markdownRendererUnderscore{}card.dat}.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{3}Runs MG5’s \markdownRendererCodeSpan{madevent} with the commands\markdownRendererInterblockSeparator
{}\markdownRendererInputFencedCode{md-cache/b9966ada17fbb7d2128a66f463428d54.verbatim}{text}{text}\markdownRendererInterblockSeparator
{}to shower the UFO events with Pythia8 and then simulate detector response with Delphes.\markdownRendererOlItemEnd 
\markdownRendererOlEnd \markdownRendererInterblockSeparator
{}The resulting Delphes ROOT file is stored under \markdownRendererCodeSpan{proc\markdownRendererUnderscore{}ufo\markdownRendererUnderscore{}parton\markdownRendererUnderscore{}ttbar/Events/ufo\markdownRendererUnderscore{}parton/} and the first \markdownRendererCodeSpan{tag\markdownRendererUnderscore{}*\markdownRendererUnderscore{}delphes*.root} is copied into\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererCodeSpan{/output/dataset/output/dataset/ufo\markdownRendererUnderscore{}ttbar\markdownRendererUnderscore{}reweighted\markdownRendererUnderscore{}delphes.root}.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{4.6 ROOT to NPZ conversion}\markdownRendererInterblockSeparator
{}The last step uses \markdownRendererCodeSpan{scripts/delphes\markdownRendererUnderscore{}to\markdownRendererUnderscore{}npz.py}:\markdownRendererInterblockSeparator
{}\markdownRendererInputFencedCode{md-cache/0ad8e0659520892f22193f55ae3bfd4f.verbatim}{bash}{bash}\markdownRendererInterblockSeparator
{}This script:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Opens the \markdownRendererCodeSpan{Delphes} tree in the ROOT file with \markdownRendererCodeSpan{uproot}.\markdownRendererUlItemEnd 
\markdownRendererUlItem Reads jet, MET, electron, muon, and event-level branches using \markdownRendererCodeSpan{awkward} for jagged arrays.\markdownRendererUlItemEnd 
\markdownRendererUlItem Pads jets to \markdownRendererCodeSpan{\markdownRendererBackslash{}text\markdownRendererLeftBrace{}max\markdownRendererBackslash{}\markdownRendererUnderscore{}jets\markdownRendererRightBrace{} = 10}, electrons to \markdownRendererCodeSpan{\markdownRendererBackslash{}text\markdownRendererLeftBrace{}max\markdownRendererBackslash{}\markdownRendererUnderscore{}ele\markdownRendererRightBrace{} = 4}, and muons to \markdownRendererCodeSpan{\markdownRendererBackslash{}text\markdownRendererLeftBrace{}max\markdownRendererBackslash{}\markdownRendererUnderscore{}mu\markdownRendererRightBrace{} = 4} using zero-padding.\markdownRendererUlItemEnd 
\markdownRendererUlItem Extracts event weights and cross sections from the \markdownRendererCodeSpan{Event} branch.\markdownRendererUlItemEnd 
\markdownRendererUlItem Writes all arrays into \markdownRendererCodeSpan{ufo\markdownRendererUnderscore{}ttbar\markdownRendererUnderscore{}reweighted.npz} as compressed NumPy arrays.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd 
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingTwo{5. Dataset contents and field definitions}\markdownRendererInterblockSeparator
{}The NPZ file \markdownRendererCodeSpan{ufo\markdownRendererUnderscore{}ttbar\markdownRendererUnderscore{}reweighted.npz} contains 17 arrays. All arrays have a leading dimension of \markdownRendererInlineMath{N = 100000} events.\markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererHeadingThree{5.1 Overview of fields}\markdownRendererInterblockSeparator
{}\markdownRendererTable{}{18}{6}{dddddd}{{Field}{Shape}{Dtype}{Description}{Units}{Level}}{{\markdownRendererCodeSpan{event\markdownRendererUnderscore{}weight}}{\markdownRendererInlineMath{(N, 1)}}{float32}{Per-event weight after EFT + \markdownRendererInlineMath{K(m_{t\bar t})}}{1}{event}}{{\markdownRendererCodeSpan{event\markdownRendererUnderscore{}xs\markdownRendererUnderscore{}pb}}{\markdownRendererInlineMath{(N, 1)}}{float32}{Per-event cross section}{pb}{event}}{{\markdownRendererCodeSpan{met}}{\markdownRendererInlineMath{(N, 1)}}{float32}{Missing transverse energy \markdownRendererInlineMath{E_T^{\text{miss}}}}{GeV}{event}}{{\markdownRendererCodeSpan{met\markdownRendererUnderscore{}phi}}{\markdownRendererInlineMath{(N, 1)}}{float32}{Azimuthal angle of MET}{rad}{event}}{{\markdownRendererCodeSpan{jet\markdownRendererUnderscore{}pt}}{\markdownRendererInlineMath{(N, 10)}}{float64}{Jet transverse momentum}{GeV}{jet}}{{\markdownRendererCodeSpan{jet\markdownRendererUnderscore{}eta}}{\markdownRendererInlineMath{(N, 10)}}{float64}{Jet pseudorapidity}{1}{jet}}{{\markdownRendererCodeSpan{jet\markdownRendererUnderscore{}phi}}{\markdownRendererInlineMath{(N, 10)}}{float64}{Jet azimuthal angle}{rad}{jet}}{{\markdownRendererCodeSpan{jet\markdownRendererUnderscore{}mass}}{\markdownRendererInlineMath{(N, 10)}}{float64}{Jet invariant mass}{GeV}{jet}}{{\markdownRendererCodeSpan{jet\markdownRendererUnderscore{}btag}}{\markdownRendererInlineMath{(N, 10)}}{int64}{Jet \markdownRendererInlineMath{b}-tag flag}{0/1}{jet}}{{\markdownRendererCodeSpan{ele\markdownRendererUnderscore{}pt}}{\markdownRendererInlineMath{(N, 4)}}{float64}{Electron transverse momentum}{GeV}{lepton}}{{\markdownRendererCodeSpan{ele\markdownRendererUnderscore{}eta}}{\markdownRendererInlineMath{(N, 4)}}{float64}{Electron pseudorapidity}{1}{lepton}}{{\markdownRendererCodeSpan{ele\markdownRendererUnderscore{}phi}}{\markdownRendererInlineMath{(N, 4)}}{float64}{Electron azimuthal angle}{rad}{lepton}}{{\markdownRendererCodeSpan{ele\markdownRendererUnderscore{}q}}{\markdownRendererInlineMath{(N, 4)}}{int64}{Electron charge}{\markdownRendererInlineMath{\pm 1}}{lepton}}{{\markdownRendererCodeSpan{mu\markdownRendererUnderscore{}pt}}{\markdownRendererInlineMath{(N, 4)}}{float64}{Muon transverse momentum}{GeV}{lepton}}{{\markdownRendererCodeSpan{mu\markdownRendererUnderscore{}eta}}{\markdownRendererInlineMath{(N, 4)}}{float64}{Muon pseudorapidity}{1}{lepton}}{{\markdownRendererCodeSpan{mu\markdownRendererUnderscore{}phi}}{\markdownRendererInlineMath{(N, 4)}}{float64}{Muon azimuthal angle}{rad}{lepton}}{{\markdownRendererCodeSpan{mu\markdownRendererUnderscore{}q}}{\markdownRendererInlineMath{(N, 4)}}{int64}{Muon charge}{\markdownRendererInlineMath{\pm 1}}{lepton}}\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{5.2 Event-level fields}\markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererHeadingFour{\markdownRendererCodeSpan{event\markdownRendererUnderscore{}weight}}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Shape: \markdownRendererInlineMath{(N, 1)}.\markdownRendererUlItemEnd 
\markdownRendererUlItem Dtype: float32.\markdownRendererUlItemEnd 
\markdownRendererUlItem Meaning: per-event weight, propagated from the Delphes \markdownRendererCodeSpan{Event.Weight} branch. Given the pipeline, this weight incorporates the EFT contribution and the \markdownRendererInlineMath{m_{t\bar t}}-dependent \markdownRendererInlineMath{K}-factor.\markdownRendererUlItemEnd 
\markdownRendererUlItem Units: dimensionless.\markdownRendererUlItemEnd 
\markdownRendererUlItem Notes: weights may be positive or negative; a small fraction of events can have negative weights, which is normal in Monte Carlo simulations involving reweighting.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingFour{\markdownRendererCodeSpan{event\markdownRendererUnderscore{}xs\markdownRendererUnderscore{}pb}}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Shape: \markdownRendererInlineMath{(N, 1)}.\markdownRendererUlItemEnd 
\markdownRendererUlItem Dtype: float32.\markdownRendererUlItemEnd 
\markdownRendererUlItem Meaning: per-event cross section, from the Delphes \markdownRendererCodeSpan{Event.CrossSection} branch.\markdownRendererUlItemEnd 
\markdownRendererUlItem Units: picobarns (pb), following Delphes conventions.\markdownRendererUlItemEnd 
\markdownRendererUlItem Notes: for unweighted samples, one typically has \markdownRendererInlineMath{\sum_i w_i = \sigma_\text{tot}} in pb; here, both \markdownRendererCodeSpan{event\markdownRendererUnderscore{}xs\markdownRendererUnderscore{}pb} and \markdownRendererCodeSpan{event\markdownRendererUnderscore{}weight} are provided for flexibility.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingFour{\markdownRendererCodeSpan{met} and \markdownRendererCodeSpan{met\markdownRendererUnderscore{}phi}}\markdownRendererInterblockSeparator
{}\markdownRendererUlBegin
\markdownRendererUlItem \markdownRendererCodeSpan{met}:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Shape: \markdownRendererInlineMath{(N, 1)}, dtype float32.\markdownRendererUlItemEnd 
\markdownRendererUlItem Meaning: missing transverse energy \markdownRendererInlineMath{E_T^{\text{miss}}}.\markdownRendererUlItemEnd 
\markdownRendererUlItem Units: GeV.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererCodeSpan{met\markdownRendererUnderscore{}phi}:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Shape: \markdownRendererInlineMath{(N, 1)}, dtype float32.\markdownRendererUlItemEnd 
\markdownRendererUlItem Meaning: azimuthal angle of the MET vector.\markdownRendererUlItemEnd 
\markdownRendererUlItem Units: radians.\markdownRendererUlItemEnd 
\markdownRendererUlItem Convention: standard azimuth in the transverse plane, expected in \markdownRendererInlineMath{[-\pi, \pi)}.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererUlItemEnd 
\markdownRendererUlEnd \markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd 
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{5.3 Jet fields}\markdownRendererInterblockSeparator
{}All jet arrays have shape \markdownRendererInlineMath{(N, N_\text{jets}^{\text{max}})} with \markdownRendererInlineMath{N_\text{jets}^{\text{max}} = 10}.\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererStrongEmphasis{Origin:} Delphes \markdownRendererCodeSpan{Jet} branches, e.g. \markdownRendererCodeSpan{Jet.PT}, \markdownRendererCodeSpan{Jet.Eta}, \markdownRendererCodeSpan{Jet.Phi}, \markdownRendererCodeSpan{Jet.Mass}, and \markdownRendererCodeSpan{Jet.BTag}.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{Ordering:} Inherited from Delphes. In standard Delphes cards, jets are ordered by decreasing \markdownRendererInlineMath{p_T}, but this is not explicitly re-sorted by \markdownRendererCodeSpan{delphes\markdownRendererUnderscore{}to\markdownRendererUnderscore{}npz.py}.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{Padding:} Events with fewer than 10 jets are padded with zeros:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererInlineMath{p_T = 0}, \markdownRendererInlineMath{\eta = 0}, \markdownRendererInlineMath{\phi = 0}, \markdownRendererInlineMath{m = 0}, \markdownRendererInlineMath{b\text{tag} = 0} indicate "no jet" at that index.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererHeadingFour{\markdownRendererCodeSpan{jet\markdownRendererUnderscore{}pt}}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Shape: \markdownRendererInlineMath{(N, 10)}.\markdownRendererUlItemEnd 
\markdownRendererUlItem Dtype: float64.\markdownRendererUlItemEnd 
\markdownRendererUlItem Meaning: transverse momentum of reconstructed jets.\markdownRendererUlItemEnd 
\markdownRendererUlItem Units: GeV.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingFour{\markdownRendererCodeSpan{jet\markdownRendererUnderscore{}eta}}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Shape: \markdownRendererInlineMath{(N, 10)}.\markdownRendererUlItemEnd 
\markdownRendererUlItem Dtype: float64.\markdownRendererUlItemEnd 
\markdownRendererUlItem Meaning: pseudorapidity of jets.\markdownRendererUlItemEnd 
\markdownRendererUlItem Units: dimensionless.\markdownRendererUlItemEnd 
\markdownRendererUlItem Convention: \markdownRendererInlineMath{\eta = -\ln \tan(\theta/2)} with \markdownRendererInlineMath{\theta} the polar angle.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingFour{\markdownRendererCodeSpan{jet\markdownRendererUnderscore{}phi}}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Shape: \markdownRendererInlineMath{(N, 10)}.\markdownRendererUlItemEnd 
\markdownRendererUlItem Dtype: float64.\markdownRendererUlItemEnd 
\markdownRendererUlItem Meaning: azimuthal angle of jets.\markdownRendererUlItemEnd 
\markdownRendererUlItem Units: radians.\markdownRendererUlItemEnd 
\markdownRendererUlItem Convention: standard azimuth in the transverse plane, expected in \markdownRendererInlineMath{[-\pi, \pi)}.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingFour{\markdownRendererCodeSpan{jet\markdownRendererUnderscore{}mass}}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Shape: \markdownRendererInlineMath{(N, 10)}.\markdownRendererUlItemEnd 
\markdownRendererUlItem Dtype: float64.\markdownRendererUlItemEnd 
\markdownRendererUlItem Meaning: reconstructed invariant mass of jets.\markdownRendererUlItemEnd 
\markdownRendererUlItem Units: GeV.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingFour{\markdownRendererCodeSpan{jet\markdownRendererUnderscore{}btag}}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Shape: \markdownRendererInlineMath{(N, 10)}.\markdownRendererUlItemEnd 
\markdownRendererUlItem Dtype: int64.\markdownRendererUlItemEnd 
\markdownRendererUlItem Meaning: \markdownRendererInlineMath{b}-tag flag per jet.\markdownRendererUlItemEnd 
\markdownRendererUlItem Values: 1 for \markdownRendererInlineMath{b}-tagged jets, 0 otherwise.\markdownRendererUlItemEnd 
\markdownRendererUlItem Notes: padded jets always have \markdownRendererCodeSpan{jet\markdownRendererUnderscore{}btag = 0}.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd 
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{5.4 Electron and muon fields}\markdownRendererInterblockSeparator
{}Electron and muon arrays each have shape \markdownRendererInlineMath{(N, N_\ell^{\text{max}})} with \markdownRendererInlineMath{N_\ell^{\text{max}} = 4}.\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererStrongEmphasis{Origin:} Delphes \markdownRendererCodeSpan{Electron} and \markdownRendererCodeSpan{Muon} branches.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{Ordering:} Inherited from Delphes, typically by decreasing \markdownRendererInlineMath{p_T}.\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{Padding:} Events with fewer than 4 leptons of a given flavor are padded with zeros:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererInlineMath{p_T = 0}, \markdownRendererInlineMath{\eta = 0}, \markdownRendererInlineMath{\phi = 0}, \markdownRendererInlineMath{q = 0} indicate no lepton at that index.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererHeadingFour{Electron fields: \markdownRendererCodeSpan{ele\markdownRendererUnderscore{}pt}, \markdownRendererCodeSpan{ele\markdownRendererUnderscore{}eta}, \markdownRendererCodeSpan{ele\markdownRendererUnderscore{}phi}, \markdownRendererCodeSpan{ele\markdownRendererUnderscore{}q}}\markdownRendererInterblockSeparator
{}\markdownRendererUlBegin
\markdownRendererUlItem \markdownRendererCodeSpan{ele\markdownRendererUnderscore{}pt}:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Shape: \markdownRendererInlineMath{(N, 4)}, dtype float64.\markdownRendererUlItemEnd 
\markdownRendererUlItem Meaning: electron transverse momentum.\markdownRendererUlItemEnd 
\markdownRendererUlItem Units: GeV.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererCodeSpan{ele\markdownRendererUnderscore{}eta}:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Shape: \markdownRendererInlineMath{(N, 4)}, dtype float64.\markdownRendererUlItemEnd 
\markdownRendererUlItem Meaning: electron pseudorapidity.\markdownRendererUlItemEnd 
\markdownRendererUlItem Units: dimensionless.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererCodeSpan{ele\markdownRendererUnderscore{}phi}:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Shape: \markdownRendererInlineMath{(N, 4)}, dtype float64.\markdownRendererUlItemEnd 
\markdownRendererUlItem Meaning: electron azimuthal angle.\markdownRendererUlItemEnd 
\markdownRendererUlItem Units: radians.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererCodeSpan{ele\markdownRendererUnderscore{}q}:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Shape: \markdownRendererInlineMath{(N, 4)}, dtype int64.\markdownRendererUlItemEnd 
\markdownRendererUlItem Meaning: electron charge.\markdownRendererUlItemEnd 
\markdownRendererUlItem Units: units of \markdownRendererInlineMath{e}.\markdownRendererUlItemEnd 
\markdownRendererUlItem Values: \markdownRendererInlineMath{+1} for positrons, \markdownRendererInlineMath{-1} for electrons; 0 indicates a padded (non-existent) slot.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererUlItemEnd 
\markdownRendererUlEnd \markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingFour{Muon fields: \markdownRendererCodeSpan{mu\markdownRendererUnderscore{}pt}, \markdownRendererCodeSpan{mu\markdownRendererUnderscore{}eta}, \markdownRendererCodeSpan{mu\markdownRendererUnderscore{}phi}, \markdownRendererCodeSpan{mu\markdownRendererUnderscore{}q}}\markdownRendererInterblockSeparator
{}\markdownRendererUlBegin
\markdownRendererUlItem \markdownRendererCodeSpan{mu\markdownRendererUnderscore{}pt}:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Shape: \markdownRendererInlineMath{(N, 4)}, dtype float64.\markdownRendererUlItemEnd 
\markdownRendererUlItem Meaning: muon transverse momentum.\markdownRendererUlItemEnd 
\markdownRendererUlItem Units: GeV.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererCodeSpan{mu\markdownRendererUnderscore{}eta}:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Shape: \markdownRendererInlineMath{(N, 4)}, dtype float64.\markdownRendererUlItemEnd 
\markdownRendererUlItem Meaning: muon pseudorapidity.\markdownRendererUlItemEnd 
\markdownRendererUlItem Units: dimensionless.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererCodeSpan{mu\markdownRendererUnderscore{}phi}:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Shape: \markdownRendererInlineMath{(N, 4)}, dtype float64.\markdownRendererUlItemEnd 
\markdownRendererUlItem Meaning: muon azimuthal angle.\markdownRendererUlItemEnd 
\markdownRendererUlItem Units: radians.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererCodeSpan{mu\markdownRendererUnderscore{}q}:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Shape: \markdownRendererInlineMath{(N, 4)}, dtype int64.\markdownRendererUlItemEnd 
\markdownRendererUlItem Meaning: muon charge.\markdownRendererUlItemEnd 
\markdownRendererUlItem Units: units of \markdownRendererInlineMath{e}.\markdownRendererUlItemEnd 
\markdownRendererUlItem Values: \markdownRendererInlineMath{+1} for \markdownRendererInlineMath{\mu^+}, \markdownRendererInlineMath{-1} for \markdownRendererInlineMath{\mu^-}; 0 indicates padding.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererUlItemEnd 
\markdownRendererUlEnd \markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd 
\markdownRendererSectionEnd 
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingTwo{6. Verification and smoke tests}\markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererHeadingThree{6.1 Inspecting the NPZ structure}\markdownRendererInterblockSeparator
{}After activating the Python environment and ensuring that this project is available at \markdownRendererCodeSpan{/output/dataset}, you can inspect the NPZ file using\markdownRendererInterblockSeparator
{}\markdownRendererInputFencedCode{md-cache/f8d235d4a5f770647e69c22b5e24897c.verbatim}{bash}{bash}\markdownRendererInterblockSeparator
{}This script prints\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem the NPZ path,\markdownRendererUlItemEnd 
\markdownRendererUlItem the list of keys,\markdownRendererUlItemEnd 
\markdownRendererUlItem the inferred number of events, and\markdownRendererUlItemEnd 
\markdownRendererUlItem for each field: shape, dtype, and basic statistics (min, max, mean) and, where appropriate, the distribution of discrete values (e.g. charges, \markdownRendererInlineMath{b}-tags).\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{6.2 Plotting basic distributions}\markdownRendererInterblockSeparator
{}A plotting script \markdownRendererCodeSpan{documentation/scripts/plot\markdownRendererUnderscore{}distributions.py} is provided with this project; you can generate basic diagnostic plots, for example:\markdownRendererInterblockSeparator
{}\markdownRendererInputFencedCode{md-cache/04400b27c65acf890a4a26671c76977b.verbatim}{bash}{bash}\markdownRendererInterblockSeparator
{}Typical plots (assuming they are created under \markdownRendererCodeSpan{documentation/plots/}) include\markdownRendererInterblockSeparator
{}\markdownRendererUlBegin
\markdownRendererUlItem Leading jet \markdownRendererInlineMath{p_T} distribution:\markdownRendererParagraphSeparator
{}\markdownRendererImage{Leading jet \markdownRendererInlineMath{p_T} distribution}{../figs/plots\markdownRendererUnderscore{}documentation/leading\markdownRendererUnderscore{}jet\markdownRendererUnderscore{}pt.png}{../figs/plots_documentation/leading_jet_pt.png}{}\markdownRendererUlItemEnd 
\markdownRendererUlItem MET distribution:\markdownRendererParagraphSeparator
{}\markdownRendererImage{MET distribution}{../figs/plots\markdownRendererUnderscore{}documentation/met.png}{../figs/plots_documentation/met.png}{}\markdownRendererUlItemEnd 
\markdownRendererUlItem Event-weight distribution:\markdownRendererParagraphSeparator
{}\markdownRendererImage{Event weight distribution}{../figs/plots\markdownRendererUnderscore{}documentation/event\markdownRendererUnderscore{}weight.png}{../figs/plots_documentation/event_weight.png}{}\markdownRendererUlItemEnd 
\markdownRendererUlItem Jet multiplicity:\markdownRendererParagraphSeparator
{}\markdownRendererImage{Jet multiplicity}{../figs/plots\markdownRendererUnderscore{}documentation/jet\markdownRendererUnderscore{}multiplicity.png}{../figs/plots_documentation/jet_multiplicity.png}{}\markdownRendererUlItemEnd 
\markdownRendererUlItem Lepton multiplicity (electrons + muons):\markdownRendererParagraphSeparator
{}\markdownRendererImage{Lepton multiplicity}{../figs/plots\markdownRendererUnderscore{}documentation/lepton\markdownRendererUnderscore{}multiplicity.png}{../figs/plots_documentation/lepton_multiplicity.png}{}\markdownRendererUlItemEnd 
\markdownRendererUlEnd \markdownRendererInterblockSeparator
{}These plots provide a quick visual check that the dataset looks reasonable for EFT \markdownRendererInlineMath{t\bar t} production: typical jet multiplicities, MET tails, and weight distributions.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{6.3 Reduced-run reproduction test (conceptual)}\markdownRendererInterblockSeparator
{}To test the full pipeline on a clean installation without regenerating the entire 100k-event dataset, one can conceptually perform a reduced run:\markdownRendererInterblockSeparator
{}\markdownRendererOlBegin
\markdownRendererOlItemWithNumber{1}Set environment variables to reduce the number of events, e.g.\markdownRendererInterblockSeparator
{}\markdownRendererInputFencedCode{md-cache/869ccfa807b3fad882069ce7cb49027b.verbatim}{bash}{bash}\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{2}Run the pipeline:\markdownRendererInterblockSeparator
{}\markdownRendererInputFencedCode{md-cache/ece3c75a369b29c0c88194769bc65e3b.verbatim}{bash}{bash}\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{3}Inspect the new NPZ and compare with the reference:\markdownRendererInterblockSeparator
{}\markdownRendererInputFencedCode{md-cache/c3809ef778c446be0586395eb30d72d1.verbatim}{bash}{bash}\markdownRendererOlItemEnd 
\markdownRendererOlItemWithNumber{4}Compare summary statistics (mean MET, mean leading jet \markdownRendererInlineMath{p_T}, etc.) and distribution shapes to those from the reference dataset, allowing for statistical fluctuations.\markdownRendererOlItemEnd 
\markdownRendererOlEnd \markdownRendererInterblockSeparator
{}This test validates that the MG5\markdownRendererUnderscore{}aMC + Pythia8 + Delphes stack and the Python environment are correctly configured.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd 
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingTwo{7. Validity regime, use cases, and limitations}\markdownRendererInterblockSeparator
{}\markdownRendererSectionBegin
\markdownRendererHeadingThree{7.1 Included physics and intended use}\markdownRendererInterblockSeparator
{}The dataset is well suited for:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Studies of EFT effects in \markdownRendererInlineMath{t\bar t} production with a non-zero chromomagnetic operator \markdownRendererInlineMath{c_{tG}}.\markdownRendererUlItemEnd 
\markdownRendererUlItem Machine-learning applications (classification and regression) using Delphes-level objects (jets, leptons, MET) and event weights.\markdownRendererUlItemEnd 
\markdownRendererUlItem Benchmarking reconstruction algorithms and simplified analyses that do not require full detector or background modeling.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}Relevant physics ingredients:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem LO matrix elements for SM and EFT \markdownRendererInlineMath{pp \to t\bar t}.\markdownRendererUlItemEnd 
\markdownRendererUlItem SM NLO corrections approximated by an \markdownRendererInlineMath{m_{t\bar t}}-dependent \markdownRendererInlineMath{K}-factor.\markdownRendererUlItemEnd 
\markdownRendererUlItem Pythia8 parton showering and hadronization.\markdownRendererUlItemEnd 
\markdownRendererUlItem Delphes 3.5.0 fast detector simulation with a standard MG5-supplied card.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{7.2 Limitations and caveats}\markdownRendererInterblockSeparator
{}Users should be aware of the following limitations:\markdownRendererInterblockSeparator
{}\markdownRendererUlBegin
\markdownRendererUlItem \markdownRendererStrongEmphasis{Approximate NLO effects:}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem The EFT UFO sample is LO in QCD; NLO QCD effects are approximated by a one-dimensional \markdownRendererInlineMath{K(m_{t\bar t})} derived from SM LO and NLO samples.\markdownRendererUlItemEnd 
\markdownRendererUlItem Correlations beyond \markdownRendererInlineMath{m_{t\bar t}} (e.g. in jet multiplicities, angular variables) are not modeled at NLO accuracy.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{EFT-specific assumptions:}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Only one dim-6 operator (\markdownRendererInlineMath{c_{tG}}) is non-zero in the DIM6 block; other Wilson coefficients are set to zero.\markdownRendererUlItemEnd 
\markdownRendererUlItem The applicability of SM-derived \markdownRendererInlineMath{K}-factors to EFT kinematics is an assumption and has not been validated beyond the one-dimensional \markdownRendererInlineMath{m_{t\bar t}} comparison.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{Top mass and width mismatch:}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem SM and EFT samples use slightly different \markdownRendererInlineMath{m_t} and \markdownRendererInlineMath{\Gamma_t}, which could introduce small shape differences unrelated to EFT effects.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{No backgrounds:}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem The dataset contains only signal \markdownRendererInlineMath{t\bar t} events with EFT contributions; no SM background processes are included.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{Detector modeling:}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem Detector response is modeled by Delphes 3.5.0 with a standard card; there is no full GEANT-based simulation and no explicit pileup modeling.\markdownRendererUlItemEnd 
\markdownRendererUlItem Performance metrics derived from this dataset are not directly comparable to full experimental analyses.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererStrongEmphasis{Reproducibility:}\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem The documentation lists explicit generator versions and reasonable Python package versions, but exact internal states (random seeds, compiler versions, parallelization details) are not fully controlled.\markdownRendererUlItemEnd 
\markdownRendererUlItem All run cards set \markdownRendererCodeSpan{iseed = 0}, allowing MadGraph5\markdownRendererUnderscore{}aMC to choose random seeds automatically; for strict bitwise determinism, one would need to fix \markdownRendererCodeSpan{iseed} explicitly in the run cards.\markdownRendererUlItemEnd 
\markdownRendererUlItem Regenerated datasets will be statistically consistent but not bit-identical.\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererUlItemEnd 
\markdownRendererUlEnd \markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingThree{7.3 Summary}\markdownRendererInterblockSeparator
{}This dataset provides a controlled and well-documented environment for studying EFT effects in \markdownRendererInlineMath{pp \to t\bar t} at 13 TeV with a non-zero chromomagnetic operator \markdownRendererInlineMath{c_{tG}}, including parton shower and fast detector simulation. It is designed for analyses that emphasize qualitative and semi-quantitative behavior rather than precision phenomenology. Users should account for the approximations and limitations described above when interpreting results.
\markdownRendererSectionEnd 
\markdownRendererSectionEnd 
\markdownRendererSectionEnd \markdownRendererDocumentEnd

==> md-cache/de809f1c5716e9d8304a034f33267dc5.md.tex <==
\markdownRendererDocumentBegin
\markdownRendererSectionBegin
\markdownRendererSectionBegin
\markdownRendererHeadingTwo{Physical process and setup}\markdownRendererInterblockSeparator
{}This dataset is a Delphes-level effective-field-theory (EFT) sample of top–antitop production at the LHC. The hard process is\markdownRendererParagraphSeparator
{}\markdownRendererDisplayMath{pp \to t\bar t}\markdownRendererParagraphSeparator
{}at a center-of-mass energy \markdownRendererInlineMath{\sqrt{s} = 13\,\text{TeV}}, generated with MadGraph5\markdownRendererUnderscore{}aMC@NLO 3.7.0, interfaced to Pythia8 for parton showering and hadronization and to Delphes 3.5.0 for fast detector simulation. The EFT model is \markdownRendererCodeSpan{dim6top\markdownRendererUnderscore{}LO\markdownRendererUnderscore{}UFO} with \markdownRendererCodeSpan{DIM6=1} and \markdownRendererCodeSpan{FCNC=0}. In the DIM6 block of the UFO param card the EFT scale is set to \markdownRendererInlineMath{\lambda = 1\,\text{TeV}} and, among the listed Wilson coefficients, only the chromomagnetic operator coefficient \markdownRendererInlineMath{c_{tG}} is non-zero; all other entries in that block are set to zero.\markdownRendererParagraphSeparator
{}Three MG5 processes are used internally: SM LO and SM NLO \markdownRendererInlineMath{pp \to t\bar t} samples (for constructing an \markdownRendererInlineMath{m_{t\bar t}}-dependent \markdownRendererInlineMath{K}-factor) and a LO EFT UFO \markdownRendererInlineMath{pp \to t\bar t} sample used for the final dataset.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingTwo{Dataset contents and observables}\markdownRendererInterblockSeparator
{}The main artifact is the NumPy archive\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererCodeSpan{/output/dataset/output/dataset/ufo\markdownRendererUnderscore{}ttbar\markdownRendererUnderscore{}reweighted.npz},\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}containing \markdownRendererInlineMath{N = 100000} events. Arrays are fixed-shape; the leading dimension is always the event index, and trailing dimensions correspond to object multiplicities with zero-padding where no object is present.\markdownRendererParagraphSeparator
{}Event-level fields:\markdownRendererInterblockSeparator
{}\markdownRendererUlBeginTight
\markdownRendererUlItem \markdownRendererCodeSpan{event\markdownRendererUnderscore{}weight} (per-event weight after EFT + \markdownRendererInlineMath{K(m_{t\bar t})} reweighting),\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererCodeSpan{event\markdownRendererUnderscore{}xs\markdownRendererUnderscore{}pb} (per-event cross section in pb),\markdownRendererUlItemEnd 
\markdownRendererUlItem \markdownRendererCodeSpan{met}, \markdownRendererCodeSpan{met\markdownRendererUnderscore{}phi} (missing transverse energy and its azimuthal angle).\markdownRendererUlItemEnd 
\markdownRendererUlEndTight \markdownRendererInterblockSeparator
{}Jet-level fields (up to 10 jets per event): \markdownRendererCodeSpan{jet\markdownRendererUnderscore{}pt}, \markdownRendererCodeSpan{jet\markdownRendererUnderscore{}eta}, \markdownRendererCodeSpan{jet\markdownRendererUnderscore{}phi}, \markdownRendererCodeSpan{jet\markdownRendererUnderscore{}mass}, \markdownRendererCodeSpan{jet\markdownRendererUnderscore{}btag}. Lepton-level fields (up to 4 electrons and 4 muons) are given by \markdownRendererCodeSpan{ele\markdownRendererUnderscore{}pt}, \markdownRendererCodeSpan{ele\markdownRendererUnderscore{}eta}, \markdownRendererCodeSpan{ele\markdownRendererUnderscore{}phi}, \markdownRendererCodeSpan{ele\markdownRendererUnderscore{}q} and \markdownRendererCodeSpan{mu\markdownRendererUnderscore{}pt}, \markdownRendererCodeSpan{mu\markdownRendererUnderscore{}eta}, \markdownRendererCodeSpan{mu\markdownRendererUnderscore{}phi}, \markdownRendererCodeSpan{mu\markdownRendererUnderscore{}q}. Units follow standard collider conventions: GeV for \markdownRendererInlineMath{p_T}, masses, and MET; radians for \markdownRendererInlineMath{\phi}; dimensionless for \markdownRendererInlineMath{\eta} and weights.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingTwo{Generation and reproducibility}\markdownRendererInterblockSeparator
{}SM LO and NLO \markdownRendererInlineMath{pp \to t\bar t} samples are used to build a one-dimensional \markdownRendererInlineMath{m_{t\bar t}}-dependent \markdownRendererInlineMath{K}-factor,\markdownRendererParagraphSeparator
{}\markdownRendererDisplayMath{K(m_{t\bar t}) = \frac{\mathrm{d}\sigma_\text{NLO}/\mathrm{d}m_{t\bar t}}{\mathrm{d}\sigma_\text{LO}/\mathrm{d}m_{t\bar t}}}\markdownRendererParagraphSeparator
{}from binned event counts in \markdownRendererInlineMath{m_{t\bar t}}. A LO EFT UFO sample is then reweighted event-by-event via\markdownRendererParagraphSeparator
{}\markdownRendererDisplayMath{w_\text{new}(m_{t\bar t}) = w_\text{orig}\,K(m_{t\bar t}),}\markdownRendererParagraphSeparator
{}and the reweighted LHE is passed through Pythia8 and Delphes. The Delphes ROOT file is converted to the NPZ file by \markdownRendererCodeSpan{scripts/delphes\markdownRendererUnderscore{}to\markdownRendererUnderscore{}npz.py}. The companion \markdownRendererCodeSpan{documentation.md} describes the full MG5\markdownRendererUnderscore{}aMC, LHAPDF 6.5.5, Pythia8, Delphes, and Python (NumPy/Awkward/Uproot) setup and provides explicit shell commands for environment installation and reduced-statistics regeneration.\markdownRendererParagraphSeparator
{}All run cards use \markdownRendererCodeSpan{iseed = 0}, letting MG5\markdownRendererUnderscore{}aMC choose random seeds automatically; reruns of the full pipeline will be statistically consistent but not bitwise-identical.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingTwo{Intended use and limitations}\markdownRendererInterblockSeparator
{}The dataset is intended for method development and exploratory studies, including EFT-sensitive analyses using jets, leptons, and MET, machine-learning applications (classification or regression on Delphes-level kinematics), and investigations of how a non-zero \markdownRendererInlineMath{c_{tG}} modifies \markdownRendererInlineMath{t\bar t} distributions.\markdownRendererParagraphSeparator
{}Limitations include: only one non-zero dim-6 operator (\markdownRendererInlineMath{c_{tG}}); no separate SM-only or background NPZ samples; NLO QCD effects approximated by a one-dimensional SM-based \markdownRendererInlineMath{K(m_{t\bar t})} rather than a full NLO+PS EFT calculation; and Delphes fast simulation without pileup or full detector effects. Systematic variations are not propagated into the NPZ, and exact bitwise reproducibility is not guaranteed. For full details, equations, and field-by-field definitions, see \markdownRendererCodeSpan{documentation.md}.
\markdownRendererSectionEnd 
\markdownRendererSectionEnd \markdownRendererDocumentEnd

==> md-cache/frozenCache.tex <==
\expandafter\global\expandafter\def\csname markdownFrozenCache0\endcsname{\input{md-cache/de809f1c5716e9d8304a034f33267dc5.md.tex}\relax}
\expandafter\global\expandafter\def\csname markdownFrozenCache1\endcsname{\input{md-cache/5a9603164a587e7211959776206a7e6c.md.tex}\relax}
\expandafter\global\expandafter\def\csname markdownFrozenCache2\endcsname{\input{md-cache/9b75a80ea0d821fdecca71e638cb1618.md.tex}\relax}

